Demand Privacy in Hotplug Caching Systems

Coded caching, introduced by Maddah-Ali and Niesen (MAN), is a model where a server broadcasts multicast packets to users with a local cache that is leveraged so as to reduce the peak network communication load. The original MAN model does not consider missing demands (i.e., some users may not request a file) or privacy issues (i.e., decoding the multicast packets may expose the users' demands). The former issue was captured by the hotplug model with offline users, where the server starts sending multicast packets after having received a certain number of file requests. The latter issue was addressed by devoting part of the cache to store privacy keys to help users decode their requested file while remaining completely ignorant about the demands of the remaining users. This paper investigates the problem of private demands against colluding users in the hotplug model with offline users. Two achievable schemes are proposed based on Maximum Distance Separable (MDS) codes. They achieve lower subpacketization, and lower load in the small memory regime compared to baseline schemes that trivially include demand privacy or offline users in known schemes.

==> ieeemacro.tex <==



\newcommand{\Bv}{{\mathbf B}}


\newcommand{\CC}{{\mathbb C}}
\newcommand{\PP}{{\mathbb P}}
\newcommand{\RR}{{\mathbb R}}
\newcommand{\QQ}{{\mathbb Q}}
\newcommand{\ZZ}{{\mathbb Z}}
\newcommand{\FF}{{\mathbb F}}
\newcommand{\GG}{{\mathbb G}}
\newcommand{\EE}{{\mathbb E}}
\newcommand{\NN}{{\mathbb N}}
\newcommand{\KK}{{\mathbb K}}


\newcommand{\av}{{\mathbf a}}
\newcommand{\bv}{{\mathbf b}}
\newcommand{\cv}{{\mathbf c}}
\newcommand{\dv}{{\mathbf d}}
\newcommand{\ev}{{\mathbf e}}
\newcommand{\fv}{{\mathbf f}}
\newcommand{\gv}{{\mathbf g}}
\newcommand{\hv}{{\mathbf h}}
\newcommand{\iv}{{\mathbf i}}
\newcommand{\jv}{{\mathbf j}}
\newcommand{\kv}{{\mathbf k}}
\newcommand{\lv}{{\mathbf l}}
\newcommand{\mv}{{\mathbf m}}
\newcommand{\nv}{{\mathbf n}}
\newcommand{\ov}{{\mathbf o}}
\newcommand{\pv}{{\mathbf p}}
\newcommand{\qv}{{\mathbf q}}
\newcommand{\rv}{{\mathbf r}}
\newcommand{\sv}{{\mathbf s}}
\newcommand{\tv}{{\mathbf t}}
\newcommand{\uv}{{\mathbf u}}
\newcommand{\wv}{{\mathbf w}}
\newcommand{\vv}{{\mathbf v}}
\newcommand{\xv}{{\mathbf x}}
\newcommand{\yv}{{\mathbf y}}
\newcommand{\zv}{{\mathbf z}}
\newcommand{\zerov}{{\mathbf 0}}
\newcommand{\onev}{{\mathbf 1}}


\newcommand{\Am}{{\mathbf A}}
\newcommand{\Bm}{{\mathbf B}}
\newcommand{\Cm}{{\mathbf C}}
\newcommand{\Dm}{{\mathbf D}}
\newcommand{\Em}{{\mathbf E}}
\newcommand{\Fm}{{\mathbf F}}
\newcommand{\Gm}{{\mathbf G}}
\newcommand{\Hm}{{\mathbf H}}
\newcommand{\Id}{{\mathbf I}}
\newcommand{\Jm}{{\mathbf J}}
\newcommand{\Km}{{\mathbf K}}
\newcommand{\Lm}{{\mathbf L}}
\newcommand{\Mm}{{\mathbf M}}
\newcommand{\Nm}{{\mathbf N}}
\newcommand{\Om}{{\mathbf O}}
\newcommand{\Pm}{{\mathbf P}}
\newcommand{\Qm}{{\mathbf Q}}
\newcommand{\Rm}{{\mathbf R}}
\newcommand{\Sm}{{\mathbf S}}
\newcommand{\Tm}{{\mathbf T}}
\newcommand{\Um}{{\mathbf U}}
\newcommand{\Wm}{{\mathbf W}}
\newcommand{\Vm}{{\mathbf V}}
\newcommand{\Xm}{{\mathbf X}}
\newcommand{\Ym}{{\mathbf Y}}
\newcommand{\Zm}{{\mathbf Z}}


\newcommand{\Ac}{{\magenta \mathcal A}}
\newcommand{\Bc}{{\mathcal B}}
\newcommand{\Cc}{{\mathcal C}}
\newcommand{\Dc}{{\mathcal D}}
\newcommand{\Ec}{{\mathcal E}}
\newcommand{\Fc}{{\mathcal F}}
\newcommand{\Gc}{{\mathcal G}}
\newcommand{\Hc}{{\mathcal H}}
\newcommand{\Ic}{{\mathcal I}}
\newcommand{\Jc}{{\mathcal J}}
\newcommand{\Kc}{{\mathcal K}}
\newcommand{\Lc}{{\blue \mathcal L}}
\newcommand{\Mc}{{\mathcal M}}
\newcommand{\Nc}{{\mathcal N}}
\newcommand{\Oc}{{\mathcal O}}
\newcommand{\Pc}{{\mathcal P}}
\newcommand{\Qc}{{\mathcal Q}}
\newcommand{\Rc}{{\mathcal R}}
\newcommand{\Sc}{{\mathcal S}}
\newcommand{\Tc}{{\mathcal T}}
\newcommand{\Uc}{{\mathcal U}}
\newcommand{\Wc}{{\mathcal W}}
\newcommand{\Vc}{{\mathcal V}}
\newcommand{\Xc}{{\mathcal X}}
\newcommand{\Yc}{{\mathcal Y}}
\newcommand{\Zc}{{\mathcal Z}}


\newcommand{\alphav}{\hbox{\boldmath$\alpha$}}
\newcommand{\betav}{\hbox{\boldmath$\beta$}}
\newcommand{\gammav}{\hbox{\boldmath$\gamma$}}
\newcommand{\deltav}{\hbox{\boldmath$\delta$}}
\newcommand{\etav}{\hbox{\boldmath$\eta$}}
\newcommand{\lambdav}{\hbox{\boldmath$\lambda$}}
\newcommand{\epsilonv}{\hbox{\boldmath$\epsilon$}}
\newcommand{\nuv}{\hbox{\boldmath$\nu$}}
\newcommand{\muv}{\hbox{\boldmath$\mu$}}
\newcommand{\zetav}{\hbox{\boldmath$\zeta$}}
\newcommand{\phiv}{\hbox{\boldmath$\phi$}}
\newcommand{\psiv}{\hbox{\boldmath$\psi$}}
\newcommand{\thetav}{\hbox{\boldmath$\theta$}}
\newcommand{\tauv}{\hbox{\boldmath$\tau$}}
\newcommand{\omegav}{\hbox{\boldmath$\omega$}}
\newcommand{\xiv}{\hbox{\boldmath$\xi$}}
\newcommand{\sigmav}{\hbox{\boldmath$\sigma$}}
\newcommand{\piv}{\hbox{\boldmath$\pi$}}
\newcommand{\rhov}{\hbox{\boldmath$\rho$}}
\newcommand{\Gammam}{\hbox{\boldmath$\Gamma$}}
\newcommand{\Lambdam}{\hbox{\boldmath$\Lambda$}}
\newcommand{\Deltam}{\hbox{\boldmath$\Delta$}}
\newcommand{\Sigmam}{\hbox{\boldmath$\Sigma$}}
\newcommand{\Phim}{\hbox{\boldmath$\Phi$}}
\newcommand{\Pim}{\hbox{\boldmath$\Pi$}}
\newcommand{\Psim}{\hbox{\boldmath$\Psi$}}
\newcommand{\Thetam}{\hbox{\boldmath$\Theta$}}
\newcommand{\Omegam}{\hbox{\boldmath$\Omega$}}
\newcommand{\Xim}{\hbox{\boldmath$\Xi$}}



\newcommand{\asf}{{\mathsf a}}
\newcommand{\bsf}{{\mathsf b}}
\newcommand{\csf}{{\mathsf c}}
\newcommand{\dsf}{{\mathsf d}}
\newcommand{\esf}{{\mathsf e}}
\newcommand{\fsf}{{\mathsf f}}
\newcommand{\gsf}{{\mathsf g}}
\newcommand{\hsf}{{\mathsf h}}
\newcommand{\isf}{{\mathsf i}}
\newcommand{\jsf}{{\mathsf j}}
\newcommand{\ksf}{{\mathsf k}}
\newcommand{\lsf}{{\mathsf l}}
\newcommand{\msf}{{\mathsf m}}
\newcommand{\nsf}{{\mathsf n}}
\newcommand{\osf}{{\mathsf o}}
\newcommand{\psf}{{\mathsf p}}
\newcommand{\qsf}{{\mathsf q}}
\newcommand{\rsf}{{\mathsf r}}
\newcommand{\ssf}{{\mathsf s}}
\newcommand{\tsf}{{\mathsf t}}
\newcommand{\usf}{{\mathsf u}}
\newcommand{\wsf}{{\mathsf w}}
\newcommand{\vsf}{{\mathsf v}}
\newcommand{\xsf}{{\mathsf x}}
\newcommand{\ysf}{{\mathsf y}}
\newcommand{\zsf}{{\mathsf z}}


\newcommand{\Asf}{{\mathsf A}}
\newcommand{\Bsf}{{\mathsf B}}
\newcommand{\Csf}{{\mathsf C}}
\newcommand{\Dsf}{{\mathsf D}}
\newcommand{\Esf}{{\mathsf E}}
\newcommand{\Fsf}{{\mathsf F}}
\newcommand{\Gsf}{{\mathsf G}}
\newcommand{\Hsf}{{\mathsf H}}
\newcommand{\Isf}{{\mathsf I}}
\newcommand{\Jsf}{{\mathsf J}}
\newcommand{\Ksf}{{\mathsf K}}
\newcommand{\Lsf}{{\mathsf L}}
\newcommand{\Msf}{{\mathsf M}}
\newcommand{\Nsf}{{\mathsf N}}
\newcommand{\Osf}{{\mathsf O}}
\newcommand{\Psf}{{\mathsf P}}
\newcommand{\Qsf}{{\mathsf Q}}
\newcommand{\Rsf}{{\mathsf R}}
\newcommand{\Ssf}{{\mathsf S}}
\newcommand{\Tsf}{{\mathsf T}}
\newcommand{\Usf}{{\mathsf U}}
\newcommand{\Wsf}{{\mathsf W}}
\newcommand{\Vsf}{{\mathsf V}}
\newcommand{\Xsf}{{\mathsf X}}
\newcommand{\Ysf}{{\mathsf Y}}
\newcommand{\Zsf}{{\mathsf Z}}


\newcommand{\sinc}{{\hbox{sinc}}}
\newcommand{\diag}{{\hbox{diag}}}
\renewcommand{\det}{{\hbox{det}}}
\newcommand{\trace}{{\hbox{tr}}}
\newcommand{\sign}{{\hbox{sign}}}
\renewcommand{\arg}{{\hbox{arg}}}
\newcommand{\var}{{\hbox{var}}}
\newcommand{\cov}{{\hbox{cov}}}
\newcommand{\SINR}{{\mathsf SINR}}
\newcommand{\SNR}{{\mathsf SNR}}
\newcommand{\Ei}{{\rm E}_{\rm i}}
\renewcommand{\Re}{{\rm Re}}
\renewcommand{\Im}{{\rm Im}}
\newcommand{\eqdef}{\stackrel{\Delta}{=}}
\newcommand{\defines}{{\,\,\stackrel{\scriptscriptstyle \bigtriangleup}{=}\,\,}}
\newcommand{\<}{\left\langle}
\renewcommand{\>}{\right\rangle}
\newcommand{\herm}{{\mathsf H}}
\newcommand{\trasp}{{\mathsf T}}
\newcommand{\transp}{{\mathsf T}}
\renewcommand{\vec}{{\rm vec}}

\newcommand{\RED}{\color[rgb]{1.00,0.10,0.10}}
\newcommand{\BLUE}{\color[rgb]{0,0,0.90}}
\newcommand{\GREEN}{\color[rgb]{0,0.80,0.20}}

\newcommand{\dt}[1]{{\red #1}}
\newcommand{\ym}[1]{{\cyan #1}}

\newtheorem{thm}{Theorem}%
\newtheorem{cor}{Corollary}
\newtheorem{lem}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{rem}{Remark}
\newtheorem{example}{Example}
\newtheorem{defn}{\protect\definitionname}

\providecommand{\definitionname}{Definition}
\providecommand{\lemmaname}{Lemma}
\providecommand{\remarkname}{Remark}
\providecommand{\theoremname}{Theorem}
